How Far Are We from Robust Voice Conversion: A Survey

Voice conversion technologies have been greatly improved in recent years with the help of deep learning, but their capabilities of producing natural sounding utterances in different conditions remain unclear. In this paper, we gave a thorough study of the robustness of known VC models. We also modified these models, such as the replacement of speaker embeddings, to further improve their performances. We found that the sampling rate and audio duration greatly influence voice conversion. All the VC models suffer from unseen data, but AdaIN-VC is relatively more robust. Also, the speaker embedding jointly trained is more suitable for voice conversion than those trained on speaker identification.

==> ForPresentation.tex <==
\begin{figure}[!h]
        \begin{subfigure}{.48\textwidth}
        \centering
        \begin{tikzpicture}[pin distance=0.08cm, scale=0.8]
            \begin{axis}[
                    xlabel={CER(\%)},
                    ylabel={SVAR(\%)},
                    xmin=-10, xmax=110,
                    ymin=-10, ymax=110,
                ]
                % Ground truth
                \node[pin=180:{\tiny VCTK}, star, black, fill, inner sep=1.5pt] at (axis cs:6.7, 97.3) {};
                \node[pin=270:{\tiny LibriTTS}, star, black, fill, inner sep=1.5pt] at (axis cs:9.5, 91.1) {};
                % AdaIN-VC
                \node[pin=0:{\tiny VCTK}, circle, red, fill, inner sep=1.5pt] at (axis cs: 37.6, 88.5) {};
                \node[pin=270:{\tiny LibriTTS}, circle, red, fill, inner sep=1.5pt] at (axis cs: 32.9, 86.5) {};
                % AutoVC red star
                \node[pin=0:{\tiny VCTK}, kite, blue, fill, inner sep=1.5pt] at (axis cs:20.8, 58.4) {};
                \node[pin=0:{\tiny LibriTTS}, kite, blue, fill, inner sep=1.5pt] at (axis cs:52.1, 9.6) {};
                
                % AutoVC + Vvec green circle
                \node[pin=90:{\tiny VCTK}, trapezium, green, fill, inner sep=1.5pt] at (axis cs: 29.3, 92.2) {};
                \node[pin=90:{\tiny LibirTTS}, trapezium, green, fill, inner sep=1.5pt] at (axis cs: 38.7, 62.6) {};
                
            \end{axis}
            \node [draw,fill=white] at (rel axis cs: 0.825, 0.852) {
            \begin{tikzpicture}
                \node[label=0:{\tiny Ground truth}, star, black, fill, inner sep=1.5pt] at (0, 1) {};
                \node[label=0:{\tiny AdaIN-VC}, circle, red, fill, inner sep=1.5pt] at (0, 0.75) {};
                \node[label=0:{\tiny \textsc{AutoVC}}, kite, blue, fill, inner sep=1.5pt] at (0, 0.5) {};
                \node[label=0:{\tiny \textsc{AutoVC}-Vvec}, trapezium, green, fill, inner sep=1.5pt] at (0, 0.25) {}; 
            \end{tikzpicture}
            };
        \end{tikzpicture}
        \vspace{-0.7em}
        \vspace{1em}
        \label{fig:AutoVC modifications}
    \end{subfigure}
\end{figure}
